PEARL: Input-Agnostic Prompt Enhancement with Negative Feedback Regulation for Class-Incremental Learning

Class-incremental learning (CIL) aims to continuously introduce novel categories into a classification system without forgetting previously learned ones, thus adapting to evolving data distributions. Researchers are currently focusing on leveraging the rich semantic information of pre-trained models (PTMs) in CIL tasks. Prompt learning has been adopted in CIL for its ability to adjust data distribution to better align with pre-trained knowledge. This paper critically examines the limitations of existing methods from the perspective of prompt learning, which heavily rely on input information. To address this issue, we propose a novel PTM-based CIL method called Input-Agnostic Prompt Enhancement with Negative Feedback Regulation (PEARL). In PEARL, we implement an input-agnostic global prompt coupled with an adaptive momentum update strategy to reduce the model's dependency on data distribution, thereby effectively mitigating catastrophic forgetting. Guided by negative feedback regulation, this adaptive momentum update addresses the parameter sensitivity inherent in fixed-weight momentum updates. Furthermore, it fosters the continuous enhancement of the prompt for new tasks by harnessing correlations between different tasks in CIL. Experiments on six benchmarks demonstrate that our method achieves state-of-the-art performance. The code is available at: https://github.com/qinyongchun/PEARL.

==> tables/alg1.tex <==
\newcommand{\INPUT}{\item[\textbf{Input:}]}
\newcommand{\TRAINone}{\item[\textbf{Phase 1:}]}
\newcommand{\TRAINtwo}{\item[\textbf{Phase 2:}]}

\begin{algorithm}[H]
\caption{ \textbf{Pseudo Code for PEARL} }
\label{alg:example}
\begin{algorithmic}[1]
\INPUT A sequence of $\mathcal{N}$ datasets $\{\mathcal{D}^1,\cdots, \mathcal{D}^{\mathcal{N}} \}$, prompt pool $\mathcal{P}$, prompt encoder $\mathbf{E}$, a memory space $\mathbf{Memory}$;

\TRAINone
\FOR{session $t$ = 1}
    \FOR{Batch in $\mathcal{D}^1$}
    \STATE Compute the global prompt $\{\texttt{[PT]}_{i}^1\}$ via Eq.~\eqref{eq:sm_1};
    \STATE Compute the logits $\Vec{l}^1$ via Eq.~\eqref{eq:sm_2};
    \STATE Optimize $\mathcal{P}$ and $\mathbf{E}$ via Eq.~\eqref{eq:sm_3};
    \ENDFOR
    \STATE Initilize memory by $\mathbf{Memory}=\{\texttt{[PT]}_{i}^1\}$
\ENDFOR

\TRAINtwo
\FOR{session $t$ = 2,$\cdots$, $\mathcal{N}$}
    \STATE Initilize $\tau=0$ and $\alpha^{\tau}=0.99$;
    \FOR{Batch in $\mathcal{D}^t$}
    \STATE Compute the global prompt $\{\texttt{[PT]}_{i}^t\}$ via Eq.~\eqref{eq:sm_1};
    \STATE Obtain the momentum prompt $\{\texttt{[PT]}_{i}^{\mathrm{mem}}\}$ via Eq.~\eqref{eq:sm_4};
    \STATE Compute the logits $\Vec{l}^t$ via Eq.~\eqref{eq:sm_5};
    \STATE Optimize $\mathcal{P}$ and $\mathbf{E}$ via Eq.~\eqref{eq:sm_3};
    \STATE Update $\alpha^{\tau}$ via Eq.~\eqref{eq:sm_6};
    \STATE Update $\tau$ by $\tau = \tau + 1$;
    \ENDFOR
    \STATE Update memory by $\mathbf{Memory}=\{\texttt{[PT]}_{i}^{\mathrm{mem}}\}$
\ENDFOR

\end{algorithmic}\label{alg:1}
\end{algorithm}

==> tables/table10.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table*}[t]
  \centering
    \begin{tabular}{lcccccccc}
    \toprule
    Method & Metric & \multicolumn{1}{l}{IN-A-10} & \multicolumn{1}{l}{CIFAR-10} & \multicolumn{1}{l}{CUB-10} & \multicolumn{1}{l}{IN-R-5} & \multicolumn{1}{l}{IN-R-10} & \multicolumn{1}{l}{IN-R-20} & \multicolumn{1}{l}{Average}  \\
    \midrule
    \multirow{2}[2]{*}{OVOR} & $\Bar{\mathcal{A}}$    & 48.49  & 86.68  & 78.12  & 76.79  & 75.61  & 73.13  & 73.14  \\
          & $\Bar{\mathcal{F}}$    & \textbf{7.83 } & 5.25  & 8.73  & 4.88  & \textbf{5.77 } & \textbf{6.06 } & 6.42  \\
    \midrule
    \multirow{2}[2]{*}{PEARL} & $\Bar{\mathcal{A}}$    & \textbf{67.41 } & \textbf{91.11 } & \textbf{92.42 } & \textbf{82.58 } & \textbf{81.09 } & \textbf{79.11 } & \textbf{82.29 } \\
          & $\Bar{\mathcal{F}}$    & 9.42  & \textbf{4.82 } & \textbf{3.99 } & \textbf{4.25 } & 5.82  & 6.48  & \textbf{5.80 } \\
    \bottomrule
    \end{tabular}%
  \caption{Comparison with OVOR on six benchmarks.}
  \label{tab:ovorsota}%
\end{table*}%


==> tables/table11.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table*}[t]
  \centering
    \begin{tabular}{lcccccccccc}
    \toprule
    Method & Task-2 & Task-3 & Task-4 & Task-5 & Task-6 & Task-7 & Task-8 & Task-9 & Task-10 & Average \\
    \midrule
    OVOR  & 0.993  & 0.996  & 0.995  & 0.998  & 0.998  & 0.999  & 0.998  & 0.999  & 0.999  & 0.997  \\
    PEARL w/o NKA & 0.932  & 0.930  & 0.932  & 0.932  & 0.931  & 0.931  & 0.927  & 0.932  & 0.933  & 0.931  \\
    PEARL & 0.558  & 0.550  & 0.561  & 0.550  & 0.554  & 0.550  & 0.551  & 0.560  & 0.563  & 0.555  \\
    \bottomrule
    \end{tabular}%
  \caption{The cosine similarity before and after prompt updating.}
  \label{tab:ovorsim}%
\end{table*}%


==> tables/table12.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table*}[t]
  \centering
    \begin{tabular}{lccccccc}
    \toprule
    Method & CIFAR & CUB   & IN-R  & IN-A  & Omni  & VTAB  & Average \\
    \midrule
    L2P   & 8.98  & 11.19  & 11.06  & 19.52  & 16.14  & 33.22  & 16.69  \\
    CODA-Prompt & 8.63  & 8.68  & 7.80  & 5.11  & 22.91  & 7.29  & 10.07  \\
    RacPAC & 4.05  & 4.74  & 6.45  & 9.05  & 7.13  & 4.19  & 5.94  \\
    PEARL & 4.42  & 4.15  & 2.41  & 9.25  & 3.33  & 3.96  & 4.59  \\
    \bottomrule
    \end{tabular}%
  \caption{The average forgetting rate ($\Bar{\mathcal{F}}$) of multiple methods.}
  \label{tab:forget}%
\end{table*}%


==> tables/table13.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table*}[t]
  \centering
    \begin{tabular}{lcccccccccccc}
    \toprule
          & \multicolumn{2}{l}{CIFAR~20-tasks} & \multicolumn{2}{c}{CUB~20-tasks} & \multicolumn{2}{c}{IN-R~40-tasks} & \multicolumn{2}{c}{IN-A~10-tasks} & \multicolumn{2}{c}{Omni~10-tasks} & \multicolumn{2}{c}{VTAB~5-tasks} \\
    Init & $\Bar{\mathcal{A}}$    & $\mathcal{A}^{\mathcal{N}}$    & $\Bar{\mathcal{A}}$    & $\mathcal{A}^{\mathcal{N}}$    & $\Bar{\mathcal{A}}$    & $\mathcal{A}^{\mathcal{N}}$    & $\Bar{\mathcal{A}}$    & $\mathcal{A}^{\mathcal{N}}$    & $\Bar{\mathcal{A}}$    & $\mathcal{A}^{\mathcal{N}}$    & $\Bar{\mathcal{A}}$    & $\mathcal{A}^{\mathcal{N}}$ \\
     \midrule
   IN21K & \textbf{93.64 } & \textbf{89.02 } & 94.48  & 89.65  & 79.54  & 72.33  & 67.41  & 57.87  & \textbf{86.87 } & 79.68  & 96.52  & \textbf{93.02 } \\
    IN1K  & 92.96  & 88.76  & \textbf{97.31 } & \textbf{94.23 } & \textbf{80.93 } & \textbf{75.45 } & \textbf{68.33 } & \textbf{59.05 } & 86.19  & \textbf{81.61 } & \textbf{96.57 } & 93.00  \\
    \bottomrule
    \end{tabular}%
  \caption{Impact of different initial parameters on performance.}
  \label{tab:initpara}%
\end{table*}%


==> tables/table14.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table*}[t]
  \centering
    \begin{tabular}{lcccc}
    \toprule
    Method & $\Bar{\mathcal{A}}$    & $\Bar{\mathcal{F}}$    & Train Time (ms) & Infer Time (ms) \\
    \midrule
    PEARL+DPG & 91.81  & 6.43  & 129.60  & 19.36  \\
    PEARL & \textbf{94.48 } & \textbf{4.71 } & \textbf{70.60 } & \textbf{13.02 } \\
    \bottomrule
    \end{tabular}%
  \caption{Impact of instance-level prompt generation on performance.}
  \label{tab:instancelevel}%
\end{table*}%


==> tables/table3.tex <==
\begin{table}[htbp]
  \centering
    \begin{tabular}{cccccc}
    \toprule
    \multicolumn{1}{c}{\multirow{2}[2]{*}{Prompt type}} & \multirow{2}[2]{*}{Layers $L$} & \multicolumn{2}{c}{IN-A~10-tasks} & \multicolumn{2}{c}{VTAB~5-tasks} \\
        &  & $\Bar{\mathcal{A}}$    & $\mathcal{A}^{\mathcal{N}}$    & $\Bar{\mathcal{A}}$    & $\mathcal{A}^{\mathcal{N}}$ \\
    \midrule
    \multicolumn{1}{c}{\multirow{4}[1]{*}{\rotatebox{90}{\parbox[c]{1.5cm}{\centering Prompt-\\tuning}}}} 
    & 1     &       &       &       &  \\          
    & 2     &       &       &       &  \\
    & 3     &       &       &       &  \\
    & 4     &       &       &       &  \\
    \midrule
    \multicolumn{1}{c}{\multirow{4}[2]{*}{\rotatebox{90}{\parbox[c]{1.5cm}{\centering Prefix-\\tuning}}}} 
    & 1     &       &       &       &  \\
    & 2     &       &       &       &  \\
    & 3     &       &       &       &  \\
    & 4     &       &       &       &  \\
    \bottomrule
    \end{tabular}%
  \caption{Add caption}
  \label{tab:prompt}%
\end{table}%

% \begin{table}[htbp]
%   \centering
%   \caption{Add caption}
%   \begin{tabular}{cccccc}
%     \toprule
%     \multirow{2}{*}{prompt type} & \multirow{2}{*}{Layer} & \multicolumn{2}{c}{IN-A} & \multicolumn{2}{c}{VTAB} \\
%     & & $\Bar{\mathcal{A}}$ & $\mathcal{A}^{\mathcal{N}}$ & $\Bar{\mathcal{A}}$ & $\mathcal{A}^{\mathcal{N}}$ \\
%     \midrule
%     \multirow{2}{*}[2ex]{\rotatebox{90}{prompt-}} & 1 & & & & \\
%     & tuning & & & & \\
%     & 2 & & & & \\
%     & & & & & \\
%     \midrule
%     \multirow{2}{*}[2ex]{\rotatebox{90}{prefix-}} & 1 & & & & \\
%     & tuning & & & & \\
%     & 2 & & & & \\
%     & & & & & \\
%     \bottomrule
%   \end{tabular}%
%   \label{tab:addlabel}%
% \end{table}%

% \begin{table}[ht]
% \centering
% \begin{tabular}{| m{2cm} | >{\centering\arraybackslash}m{2cm} | m{2cm} |}
% \hline
% 1 & 2 & 3 \\
% \hline
% 4 & 5 & 6 \\
% \hline
% \end{tabular}
% \caption{示例表格}
% \end{table}


% \begin{tabular}{|c|c|}
% \hline
% Normal Text & \rotatebox{90}{Vertical Text} \\
% \hline
% More Text & \rotatebox{90}{Another Vertical Text} \\
% \hline
% \end{tabular}


==> tables/table6.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
    \begin{tabular}{clrr}
    \toprule
    \multicolumn{2}{c}{\multirow{2}[2]{*}{Method}} & \multicolumn{2}{c}{IN-A} \\
    \multicolumn{2}{c}{} & \multicolumn{1}{c}{$\Bar{\mathcal{A}}$    } & \multicolumn{1}{c}{$\mathcal{A}^{\mathcal{N}}$} \\
    \midrule
    \multicolumn{1}{p{6.1em}}{L2P} & w/ Momentum & 53.36  & 43.45  \\
    w/ Prompt Encoder & \cellcolor[rgb]{ .906,  .902,  .902}w/o Momentum & \cellcolor[rgb]{ .906,  .902,  .902}58.16  & \cellcolor[rgb]{ .906,  .902,  .902}49.18  \\
    \midrule
    \multicolumn{1}{p{6.1em}}{DualPrompt} & w/ Momentum & 57.05  & 46.61  \\
    w/ Prompt Encoder & \cellcolor[rgb]{ .906,  .902,  .902}w/o Momentum & \cellcolor[rgb]{ .906,  .902,  .902}60.50  & \cellcolor[rgb]{ .906,  .902,  .902}50.69  \\
    \midrule
    \multicolumn{1}{p{6.1em}}{CODA-Prompt} & w/ Momentum & 59.67  & 47.33  \\
    w/ Prompt Encoder & \cellcolor[rgb]{ .906,  .902,  .902}w/o Momentum & \cellcolor[rgb]{ .906,  .902,  .902}61.83  & \cellcolor[rgb]{ .906,  .902,  .902}51.68  \\
    \bottomrule
    \end{tabular}%

    \caption{Add caption}
  \label{tab:sm_prompt}%
\end{table}%



==> tables/table7.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[t]
  \centering
    \begin{tabular}{crlrl}
    \toprule
    \multirow{2}[2]{*}{$H$} & \multicolumn{2}{c}{IN-A 10-tasks} & \multicolumn{2}{c}{VTAB 5-tasks} \\
          & \multicolumn{1}{c}{ $\Bar{\mathcal{A}}$} & \multicolumn{1}{c}{$\mathcal{A}^{\mathcal{N}}$} & \multicolumn{1}{c}{ $\Bar{\mathcal{A}}$} & \multicolumn{1}{c}{$\mathcal{A}^{\mathcal{N}}$}  \\
    \midrule
    2   & 66.36 & 57.34 &  95.52  &  92.31 \\
    4   & 66.58 & 57.27 &  95.45  &  92.21 \\
    6   & 66.48 & \textbf{57.80} &  95.42  &  92.38 \\
    8   & 66.58 & 57.34 &  95.47  &  92.52 \\
    10   & \textbf{66.59} & 57.67 &  \textbf{95.53}   & \textbf{92.53} \\
    \bottomrule
    \end{tabular}%
   \caption{Ablation study of the length of the prompt token.}
 \label{tab:sm_layer}%
\end{table}%


==> tables/table8.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[h]
  \centering
    \begin{tabular}{crlrl}
    \toprule
    \multirow{2}[2]{*}{$H$} & \multicolumn{2}{c}{CUB 10-tasks} & \multicolumn{2}{c}{VTAB 5-tasks} \\
          & \multicolumn{1}{c}{ $\Bar{\mathcal{A}}$} & \multicolumn{1}{c}{$\mathcal{A}^{\mathcal{N}}$} & \multicolumn{1}{c}{ $\Bar{\mathcal{A}}$} & \multicolumn{1}{c}{$\mathcal{A}^{\mathcal{N}}$}  \\
    \midrule
    Learnable $g(\cdot)$     &  00.00     &   00.00    &    00.00   & 00.00 \\
    RanPAC $g(\cdot)$     &       &       &       &  \\
    \bottomrule
    \end{tabular}%
   \caption{Add caption}
 \label{tab:H}%
\end{table}%


==> tables/table9.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[t]
  \centering
    \begin{tabular}{lccc}
    \toprule
    Pool Length & $\Bar{\mathcal{A}}$    & $\mathcal{A}^{\mathcal{N}}$    & $\Bar{\mathcal{F}}$ \\
    \midrule
    20    & 66.64  & 57.80  & \textcolor[rgb]{ .267,  .447,  .769}{11.23 } \\
    50    & 66.51  & \textcolor[rgb]{ .267,  .447,  .769}{57.67 } & 10.00  \\
    100   & \textcolor[rgb]{ 1,  0,  0}{67.41 } & 57.87  & \textcolor[rgb]{ 1,  0,  0}{9.25 } \\
    200   & \textcolor[rgb]{ .267,  .447,  .769}{66.39 } & \textcolor[rgb]{ 1,  0,  0}{58.46 } & 9.59  \\
    400   & 66.78  & 58.20  & 9.98  \\
    \bottomrule
    \end{tabular}%
  \caption{Ablation study of the length of the prompt token. Red represents the best while blue represents the worst.}
  \label{tab:poolpength}%
\end{table}%

